A Faster FPTAS for #Knapsack

Given a set $W = \{w_1,\ldots, w_n\}$ of non-negative integer weights and an integer $C$, the #Knapsack problem asks to count the number of distinct subsets of $W$ whose total weight is at most $C$. In the more general integer version of the problem, the subsets are multisets. That is, we are also given a set $ \{u_1,\ldots, u_n\}$ and we are allowed to take up to $u_i$ items of weight $w_i$. We present a deterministic FPTAS for #Knapsack running in $O(n^{2.5}\varepsilon^{-1.5}\log(n \varepsilon^{-1})\log (n \varepsilon))$ time. The previous best deterministic algorithm [FOCS 2011] runs in $O(n^3 \varepsilon^{-1} \log(n\varepsilon^{-1}))$ time (see also [ESA 2014] for a logarithmic factor improvement). The previous best randomized algorithm [STOC 2003] runs in $O(n^{2.5} \sqrt{\log (n\varepsilon^{-1}) } + \varepsilon^{-2} n^2 )$ time. Therefore, in the natural setting of constant $\varepsilon$, we close the gap between the $\tilde O(n^{2.5})$ randomized algorithm and the $\tilde O(n^3)$ deterministic algorithm. For the integer version with $U = \max_i \{u_i\}$, we present a deterministic FPTAS running in $O(n^{2.5}\varepsilon^{-1.5}\log(n\varepsilon^{-1} \log U)\log (n \varepsilon) \log^2 U)$ time. The previous best deterministic algorithm [APPROX 2016] runs in $O(n^3\varepsilon^{-1}\log(n \varepsilon^{-1} \log U) \log^2 U)$ time.

==> graphics/apx/axes.tex <==
\draw [<->] (0,15) node (yaxis) [above] {$\sumof{f}(x)$}
	|- (15,0) node (xaxis) [right] {$x$};


==> graphics/apx/bludots2.tex <==
\filldraw [blue] (0,0) circle (2pt)
				(2,0) circle (6pt)
				(6,0) circle (6pt)
				(10,0) circle (8pt)
				(14,0) circle (4pt);

==> graphics/apx/blueaxes.tex <==
\draw [<->] (0,15) node (yaxis) [above, blue] {$\tildes{f}(x)$}
	|- (15,0) node (xaxis) [right] {$x$};

==> graphics/apx/bluedots.tex <==
\filldraw[blue]   	(0,1) circle (3pt)
					(2,3) circle (3pt)
					(6,6) circle (3pt)
					(10,10) circle (3pt)
					(14,13) circle (3pt);

==> graphics/apx/reddots.tex <==
\filldraw [red] (0,0) circle (2pt)
				(2,0) circle (4pt)
				(4,0) circle (2pt)
				(6,0) circle (4pt)
				(7,0) circle (2pt)
				(10,0) circle (6pt)
				(12,0) circle (2pt)
				(14,0) circle (4pt);

==> graphics/apx/sumf.tex <==
\draw 	(0,1) -- (2,1)
		(2,3) -- (4,3)
		(4,4) -- (6,4)
		(6,6) -- (7,6)
		(7,7) -- (10,7)
		(10,10) -- (12,10)
		(12,11) -- (14,11)
		(14,13) -- (15,13);

\draw[dotted] 	(2,1) -- (2,3)
				(4,3) -- (4,4)
				(6,4) -- (6,6)
				(7,6) -- (7,7)
				(10,7) -- (10,10)
				(12,10) -- (12,11)
				(14,11) -- (14,13);  

==> graphics/apx/tildes.tex <==
\begin{scope}[thick, blue]

	\draw 	(0,1) -- (2,1)
			(2,4) -- (6,4)
			(6,7) -- (10,7)
			(10,11) -- (14,11)
			(14,13) -- (15,13);

	\draw[dotted] 	(2,1) -- (2,4)
					(6,4) -- (6,7)
					(10,7) -- (10,11)
					(14,11) -- (14,13);  

\end{scope}


==> graphics/apx/xi.tex <==
\begin{scope}[below]
	\node (x1) at (0,-0.5) {$x_1$};
	\node (x2) at (2,-0.5) {$x_2$};
	\node (x3) at (2,-1.5) {$x_3$};
	\node (x4) at (6,-0.5) {$x_4$};
	\node (x5) at (10,-0.5) {$x_5$};
	\node (x6) at (14,-0.5) {$x_6$};
\end{scope}
